Selberg, Ihara and Berkovich

We use the Selberg zeta function to study the limit behavior of resonances in a degenerating family of Kleinian Schottky groups. We prove that, after a suitable rescaling, the Selberg zeta functions converge to the Ihara zeta function of a limiting finite graph associated to the relevant non-Archimedean Schottky group acting on the Berkovich projective line. Moreover, we show that these techniques can be used to get an exponential error term in a result of McMullen (recently extended by Dang and Mehmeti) about the asymptotics for the vanishing rate of the Hausdorff dimension of limit sets of certain degenerating Schottky groups generating symmetric three-funnel surfaces. Here, one key idea is to introduce an intermediate zeta function capturing \emph{both} non-Archimedean and Archimedean information (while the traditional Selberg, resp. Ihara zeta functions concern only Archimedean, resp. non-Archimedean properties).

==> file/speed-old.tex <==
\section{Speed of convergence}
\subsection{Laurent expansion of traces}

In order to study the speed of convergence, we need a more precise expansion of the euclidean length. We make use of the Fricke relation of $\SL_2$, that is for $g,h\in\SL_2 $
\begin{equation}\label{equ:fricke}
\tr(gh)+\tr(gh^{-1})=\tr(g)\tr(h).
\end{equation}
Then we study the trace of a word through the geometry of Schottky groups. \olive{Currently, I only know how to prove the two generator case. This method seems not easy to be generalized to more generators situation. The use of \cref{equ:fricke} is not very important. We may also use the parameters $\alpha_j,\beta_j,\lambda_j$ in the definition of Schottky groups directly to obtain upper bound of coefficients. But the lower bound of the coefficient of the leading term is hard to get.}
\begin{prop}\label{prop:laurent}
    Let $\Gamma$ be a non-archimedean Schottky of two generators. We can find generators $\gamma_1,\gamma_2$ such that the following holds: Let
    \[\tr(\gamma_1)=At^{-n_1}+\cdots,\ \tr(\gamma_2)=Bt^{-n_2}+\cdots,\ \tr(\gamma_1\gamma_2)=Dt^{-n_3}+\cdots,  \]
    with $A,B,D$ non-zero. Then either $n_3\neq n_1+n_2$ or $n_3=n_1+n_2$ and $D-AB\neq 0$.
    
    Moreover, for any word $w=\gamma_{a_1}\cdots\gamma_{a_m}$, we have
    \[ \tr(w)=t^{-\ell^{na}(w)}(A_0+A_1t+\cdots), \]
    with $A_0$ a monomial on $A,B,D$ with integral coefficient (and possible $D-AB$ when $n_3=n_1+n_2$), and $|A_j|=O(e^{(Cm+j)})$. The constant $C$ only depends on the Schottky group.
\end{prop}

\begin{proof}
If $n_1+n_2=n_3$ and $AB-D=0$, then we change the choice of generator. Consider
\[\tr(\gamma_1)=At^{-n_1}+\cdots,\ \tr(\gamma_2^{-1})=Bt^{-n_2}+\cdots,\ \tr(\gamma_1\gamma_2^{-1})=D't^{-n_3'}+\cdots.  \]
Since $\tr(\gamma_1\gamma_2^{-1})=\tr(\gamma_1)\tr(\gamma_2)-\tr(\gamma_1\gamma_2) $, we know that $n_3'<n_1+n_2$ and we are in the desired situation.


By \cref{equ:fricke}, we can express $\tr(w)$ as a polynomial $P_w$ on three variables $\tr(\gamma_1),\tr(\gamma_2)$ and $\tr(\gamma_1\gamma_2)$ with integral coefficients. This polynomial $P_w$ only depends on the word $w$. Due to the definition of Schottky groups, the entries are in the Banach ring $A_r$ with finite hybrid norm, we know that the coefficients of $\tr(\gamma_1),\tr(\gamma_2)$ and $\tr(\gamma_1\gamma_2)$ on $t$ grow slower than $e^n$. From these, we obtain the bound on $|A_j|$. This is easier to see from $\tr(w)=\tr(\gamma_{a_1}\cdots\gamma_{a_m})$. The trace $\tr(w)$ is at most a sum of $4^m$ terms of $m$-product of entries of $\gamma_i$, with each term in $A_r$. Then we use the hypbrid norm being sub multiplicative to conclude.

For the coefficient $A_0$, we know it is a polynomial on $A,B,D$, because $A_0$ is the coefficicent of the lower ordre term of the polynomial \[P_w(\tr(\gamma_1),\tr(\gamma_2),\tr(\gamma_1\gamma_2))=P_w(At^{-n_1}+\cdots,Bt^{-n_2}+\cdots,Dt^{-n_3}+\cdots ) .\] 
If $n_1+n_2\neq n_3$, then for any choice of non-zero $A,B,D$, (all the possible choices of $A,B,D$ can be realized through Schottky groups, see \cref{exam:surj}) the skeleton $\Sigma_X$ of the Schottky group is the same graph. Because the graph is either a three regular graph with two vertices or a four regular graph with one vertex. With knowledge of the non-archimedean length of loops $\gamma_1,\gamma_2,\gamma_1\gamma_2,\gamma_1\gamma_2^{-1}$, we can uniquely determine the graph, where the length of $\gamma_1\gamma_2$ is obtain through $\tr(\gamma_1)\tr(\gamma_2)-\tr(\gamma_1\gamma_2)$ with the leading term given by $ABt^{-n_1-n_2}$ or $-Dt^{-n_3}$.

Hence the non-archimedean length $\ell^{na}(w)$, which is the length of the corresponding loop of $w$ in the graph $\Sigma_X$, stays the same. Therefore the polynomial $A_0$ is non-zero for any $(A,B,D)\in\C^3$ with $ABD\neq 0$. By basic algebraic geometry, we know that $A_0$ must be a monomial on $A,B,D$.

If $n_1+n_2=n_3$ and $AB-D\neq 0$, then the graph $\Sigma_X$ is also uniquely determined. By the same argument, we know that $A_0$ is a nomonial on $A,B,D,AB-D$.
%
\end{proof}

\begin{exam}\label{exam:surj}
    Up to conjugacy, suppose $\gamma_1$ fixes $0,\infty$ and $\gamma_2$ fixes $1,\alpha(t)$. Let $\gamma_1=\diag(At^{-n_1}, (At^{-n_1})^{-1} )$ and $\gamma_2= P\diag(Bt^{-n_2}, (Bt^{-n_2})^{-1} )P^{-1} $ with $P=\begin{pmatrix}
        \frac{1}{1-\alpha } & \alpha \\ \frac{1}{1-\alpha }& 1
    \end{pmatrix}$. Then \[\tr(\gamma_1\gamma_2)=\frac{ABt^{-n_1-n_2}}{1-\alpha}-\frac{\alpha}{1-\alpha}(AB^{-1}t^{-n_1+n_2}+A^{-1}Bt^{n_1-n_2})\]

    By choosing $1-\alpha=ABD^{-1}t^{-n_1-n_2+n_3}\in\C((t))$, we can obtain all the possible leading term $Dt^{-n_3}$. 
    
    In this situation, we have two possible values of cross-ratio, either $\alpha$ or $1/\alpha$. The contracting ratio is given by $\lambda(\gamma_1)=A^2t^{-2n_1},\ \lambda(\gamma_2)=B^2t^{-2n_2}$. We are able to verify that the order of vanishing is positive for $|n_1-n_2|<n_3$, which is a necessary condition for being Schottky.
    
    For two generator case, the traces $\tr(\gamma_1),\tr(\gamma_2),\tr(\gamma_1\gamma_2)$ give another parmatrization of the space of Schottky groups.
    %Need to verify details that this gives a Schottky family.
    %More precisely,\begin{itemize} \item for $|n_1-n_2|<n_3<n_1+n_2$, let $1-\alpha=ABD^{-1}t^{-n_1-n_2+n_3}$. \item for $n_3=n_1+n_2$, let $1-\alpha=ABD^{-1}$ \item for $n_3>n_1+n_2$, let $1-\alpha=ABD^{-1}t^{-n_1-n_2+n_3}$. \end{itemize}
\end{exam}

\paragraph{Another proof}

\olive{For the lower bound of $A_0(w)$, we can also use \cref{lem-uniform ell} and Jensen's inequality to prove.}
\begin{proof}
    By \cref{lem-uniform ell}, for any conjugacy class $[\gamma]$ with $\ell^{na}(\gamma)>1/c$ and $|t|<c$, we have
    \[\ell(\gamma_t)\geq c\log(1/|t|)\ell^{na}(\gamma). \]
    Let $\lambda_1(\gamma_t),\lambda_2(\gamma_t)$ be the two eigenvalues of $\gamma_t$ with $|\lambda_1(\gamma_t)|>1$. Notice that $\log|\lambda_1(\gamma_t)|=\ell(\gamma_t)=-\log|\lambda_2(\gamma_t)|$. For $|t|<c$
    \begin{equation}\label{equ:trgg}
     |\tr(\gamma_t)|\geq e^{\ell(\gamma_t)}-e^{-\ell(\gamma_t)}\geq \frac{1}{2}(1/|t|)^{c\ell^{na}(\gamma)}. 
    \end{equation}
    Recall
    \begin{equation}\label{equ:trgamma}
     \tr(\gamma_t)=t^{-\ell^{na}(\gamma)}(A_0+A_1t+\cdots). 
    \end{equation}
    Let $f(t)=A_0+A_1t+\cdots$, which is an analytic function on $|t|<1/e$. 
    By \cref{equ:trgg,equ:trgamma} we obtain for $|t|<c$,
    \[ \log|f(t)|\geq -(1-c)\ell^{na}(\gamma)\log(1/|t|)-\log 2. \]
    Applying mean value property to $\log|f|$, which is harmonic on $|t|<c$, on the circle $|t|=c/2$,
    \begin{align*}
     \log |A_0|&=\log|f(0)|=\int_{\R/\Z} \log |f(\frac{c}{2}e^{2\pi i\theta})|\dd\theta\\
    &\geq (c-1)\ell^{na}(\gamma)\log(2/c)-\log2.
    \end{align*}
    Therefore, we obtain an exponential lower bound of $|A_0(\gamma)|$ by its non-archimedean length.
\end{proof}


\subsection{Speed of convergence}

In this section we discuss how to get quantitative estimates on the speed of convergence. The key to get a quantitative estimate is the Hadamard three circle theorem.

\begin{prop}\label{prop:hadamard}
    Let $f(z):\{r_1 \leq |z-a| \leq r_3\}\to\mathbb{C}$ be a holomorphic function, $r_1\leq r_2\leq r_3$ and $t=\log(r_3/r_2)/\log(r_3/r_1)\in [0,1]$. Then
    \begin{equation*}
        \max_{|z-a|=r_2}|f(z)|\leq \left(\max_{|z-a|=r_1}|f(z)|\right)^{t}\left(\max_{|z-a|=r_3} |f(z)|\right)^{1-t}.
    \end{equation*}
\end{prop}
%{\olive{the version of three-circle should be $t=\log(r_3/r_2)/\log(r_3/r_1)$}}
\begin{proof}
    This follows from the fact that $\log|f(z)|$ is a subharmonic function.
\end{proof}

The strategy is to prove convergence in the region $s\gg 1$ and use Proposition~\ref{prop:hadamard} to conclude convergence in a larger region.

\begin{lem}
There exists $s_0>0$, such that for $\Re s>s_0$, we have for any $\epsilon>0$,
\begin{equation*}
        \left|\frac{Z(s/|\log t|)}{Z^{na}(s)}-1\right|\lesssim_{\epsilon} |\log t|^{-1+\epsilon}.
\end{equation*}
\end{lem}


\begin{proof}
First we deal with convergence of lengths of geodesics. \olive{Due to \cref{prop:laurent}}, for each word $w=\gamma_{a_1}\cdots\gamma_{a_m}$,

%Suppose the Schottky group has a family of generators $\gamma_a$, $\gamma_{\bar a}=\gamma_a^{-1}$, $a=1,2,\cdots,r$, with 
%\begin{equation*}
%    \gamma_a(t)=t^{-n_a} (\gamma_a^0+\cal{O}(t)).
%\end{equation*}
%\olive{we may have $\gamma_a^0$ dengenerate like $\begin{pmatrix}    0 & 1 \\ 0 & 0\end{pmatrix}$, should be more careful. Indeed, we need a more detail estimate. One to do it is to use the skeleton, the finite tree. Use \cref{prop:laurent} to rewrite this computational part. We can also keep the leading coefficient $A_0$ to obtain better error terms.}
%The length of the closed geodesic fixed by $\gamma_a$ is $\log \lambda_1(\gamma_a^0)+n_a|\log t|+\cal{O}(t)$. On the other hand, the non-Archimedean length is just $n_a$. So
%\begin{equation*}
%    \ell(\gamma_a)/|\log t| = \ell^{na}(\gamma_a)+\frac{\log \lambda_1(\gamma_a^0)}{|\log t|}+\mathcal{O}(t/|\log t|).
%\end{equation*}
%In general, since $\gamma_{a_1}\cdots\gamma_{a_m}=t^{-n_{a_1}-\cdots-n_{a_m}}(\gamma_{a_1}^0\cdots \gamma_{a_m}^0+\mathcal{O}(e^{Cm}t))$, for $m\leq |\log t|^{\epsilon}$,
\begin{equation*}
   \log \tr(w_t)/\log 1/|t|=\ell^{na}(w)+\log|A_0(w)|/\log 1/|t|+\log(1+A_1(w)t/A_0(w)+\cdots)/\log 1/|t|.
\end{equation*}
Moreover, for $|A_0(w)|$, we have a lower bound
\[ |A_0(w)|\geq C^{-m}, \]
with $C$ depending on the Schottky group. For $A_j(w)$, we have an upper bound $A_j(w)=O(e^{Cm+j})$. We also have
\[ |\log\tr(w_t)-\ell(w_t)|=\log(1+e^{-2\ell(w_t)})\ll t. \]
Therefore, 
\begin{equation}\label{equ:expansion}
\ell(w_t)/\log 1/|t|=\ell^{na}(w)+\log|A_0(w)|/\log 1/|t|+O(e^{Cm}t)/\log 1/|t|. 
\end{equation}
%Denote by \[\ell(w,t)=\ell^{na}(w)+\log|A_0(w)|/\log 1/|t|\]
Consequently, for word length $l(\gamma)\leq |\log t|^{1/2C}$ and $\Re s>1$,
\begin{equation*}
\begin{aligned}
    &\left|\log(1-e^{-s\ell(\gamma)/|\log t|})-\log (1-e^{-s\ell^{na}(\gamma)})\right|\lesssim \left| e^{-s\ell(\gamma)/|\log t|}-e^{-s\ell^{na}(\gamma)} \right|\\
    &= e^{-\Re s \ell^{na}(\gamma)}\left|1-e^{\Re s |s\ell^{na}(\gamma)-\ell(\gamma)/|\log t||}\right|\lesssim e^{-\Re s \ell^{na}(\gamma)}/\log 1/|t|,
\end{aligned}
\end{equation*} 
where the last inequality is due to \cref{equ:expansion}.

On the other hand for $\ell^{na}(\gamma)>|\log t|^{\epsilon}$, we have
\begin{equation*}
    \log(1-e^{-s\ell(\gamma)/|\log t|})+\log (1-e^{-s\ell^{na}(\gamma)})\lesssim e^{-c\Re s\ell^{na}(\gamma)}.
\end{equation*}
Thus for $\Re s$ sufficiently large, we have
\begin{equation*}
    \sum\limits_{\gamma}\log(1-e^{-s\ell(\gamma)/|\log t|})-\log (1-e^{-s\ell^{na}(\gamma)})\lesssim |\log t|^{\epsilon-1}\sum\limits_{n\leq |\log t|^{\epsilon}}e^{-\Re s \ell^{na}(\gamma)}+e^{(C-c\Re s)|\log t|^{\epsilon}}\lesssim_{\epsilon} |\log t|^{\epsilon-1}. \qedhere
\end{equation*}
\end{proof}
\olive{For general Schottky group, the logarithm rate seems optimal. But for special family (the example in \cite{pollicottZerosSelbergZeta2019a}), we may use the knowledge of coefficients $A_j(w)$ to obtain better rate. }

Recall that by Proposition~\ref{p:sing-est-3d},
\begin{equation*}
    |Z(s)|\leq\prod\limits_{\ell=0}^\infty(1+\mu_{\ell}(\mathcal{L}_s))\leq \exp\left(\sum\limits_{\ell=0}^{\infty}\mu_{\ell}(\mathcal{L}_s)\right)\leq \exp(\Tilde{C}(r,B)\exp((A+\pi)|s|)).
\end{equation*}
In our case $r$ and $B$ are fixed and $A\lesssim |\log t|$, so $Z(s/|\log t|)$ is uniformly bounded for $s$ inside any fixed disc. Proposition~\ref{prop:hadamard} then implies that
\begin{prop}
    For any $R>0$ and $\epsilon>0$, we have
    \begin{equation*}
        |Z(s/|\log t|)-Z^{na}(s)|\lesssim_{R,\epsilon} |\log t|^{-1+\epsilon},\quad |s|\leq R.
    \end{equation*}
\end{prop}

\begin{comment}
    
We introduce a middle zeta function given by
\[ Z_M(s,t)=\prod_{[\gamma]\in P}(1-e^{-s\ell(\gamma,t)}), \]
where $A_0(\gamma)$ is the coefficient of the leading term in $\tr(\gamma)$.

\begin{proof}
First we deal with convergence of lengths of geodesics. Due to \cref{prop:laurent}, for each word $w=\gamma_{a_1}\cdots\gamma_{a_m}$,

%Suppose the Schottky group has a family of generators $\gamma_a$, $\gamma_{\bar a}=\gamma_a^{-1}$, $a=1,2,\cdots,r$, with 
%\begin{equation*}
%    \gamma_a(t)=t^{-n_a} (\gamma_a^0+\cal{O}(t)).
%\end{equation*}
%\olive{we may have $\gamma_a^0$ dengenerate like $\begin{pmatrix}    0 & 1 \\ 0 & 0\end{pmatrix}$, should be more careful. Indeed, we need a more detail estimate. One to do it is to use the skeleton, the finite tree. Use \cref{prop:laurent} to rewrite this computational part. We can also keep the leading coefficient $A_0$ to obtain better error terms.}
%The length of the closed geodesic fixed by $\gamma_a$ is $\log \lambda_1(\gamma_a^0)+n_a|\log t|+\cal{O}(t)$. On the other hand, the non-Archimedean length is just $n_a$. So
%\begin{equation*}
%    \ell(\gamma_a)/|\log t| = \ell^{na}(\gamma_a)+\frac{\log \lambda_1(\gamma_a^0)}{|\log t|}+\mathcal{O}(t/|\log t|).
%\end{equation*}
%In general, since $\gamma_{a_1}\cdots\gamma_{a_m}=t^{-n_{a_1}-\cdots-n_{a_m}}(\gamma_{a_1}^0\cdots \gamma_{a_m}^0+\mathcal{O}(e^{Cm}t))$, for $m\leq |\log t|^{\epsilon}$,
\begin{equation*}
    \ell(w_t)/\log 1/|t|=\ell^{na}(w)+\log|A_0(w)|/\log 1/|t|+\log(1+A_1(w)t/A_0(w)+\cdots)/\log 1/|t|.
\end{equation*}
Moreover, for $|A_0(w)|$, we have a lower bound
\[ |A_0(w)|\geq C^{-m}, \]
with $C$ depending on the Schottky group. For $A_j(w)$, we have an upper bound $A_j(w)=O(e^{Cm+j})$. Therefore, 
\begin{equation}\label{equ:expansion}
\ell(w_t)/\log 1/|t|=\ell^{na}(w)+\log|A_0(w)|/\log 1/|t|+O(e^{Cm}t)/\log 1/|t|. 
\end{equation}
Denote by \[\ell(w,t)=\ell^{na}(w)+\log|A_0(w)|/\log 1/|t|\]
Consequently, for word length $l(\gamma)\leq |\log t|^{1/2C}$ and $\Re s>1$,
\begin{equation*}
\begin{aligned}
    &\left|\log(1-e^{-s\ell(\gamma)/|\log t|})-\log (1-e^{-s\ell(\gamma,t)})\right|\lesssim \left| e^{-s\ell(\gamma)/|\log t|}-e^{-s\ell(\gamma,t)} \right|\\
    &= e^{-\Re s \ell(\gamma,t)}\left|1-e^{\Re s |s\ell(\gamma,t)-\ell(\gamma)/|\log t||}\right|\lesssim e^{-\Re s \ell^{na}(\gamma)}||t|^{1/2},
\end{aligned}
\end{equation*} 
where the last inequality is due to \cref{equ:expansion}.

On the other hand for $\ell^{na}(\gamma)>|\log t|^{\epsilon}$, we have
\begin{equation*}
    \log(1-e^{-s\ell(\gamma)/|\log t|})+\log (1-e^{-s\ell^{na}(\gamma)})\lesssim e^{-c\Re s\ell^{na}(\gamma)}.
\end{equation*}
Thus for $\Re s$ sufficiently large, we have
\begin{equation*}
    \sum\limits_{\gamma}\log(1-e^{-s\ell(\gamma)/|\log t|})-\log (1-e^{-s\ell^{na}(\gamma)})\lesssim |\log t|^{\epsilon-1}\sum\limits_{n\leq |\log t|^{\epsilon}}e^{-\Re s \ell^{na}(\gamma)}+e^{(C-c\Re s)|\log t|^{\epsilon}}\lesssim_{\epsilon} |\log t|^{\epsilon-1}. \qedhere
\end{equation*}
\end{proof}

\end{comment}

==> macros.tex <==
\RequirePackage{extarrows}
\RequirePackage{mathtools}
\RequirePackage{textcomp}
\RequirePackage{wasysym}
\RequirePackage{tikz}
\usetikzlibrary{decorations.markings}
\RequirePackage{graphicx}
\usetikzlibrary{arrows}
\usetikzlibrary{calc}
\usepackage{esint}

\newcommand{\highlight}[1]{{\color{magenta} #1}}
\newcommand{\significant}[1]{\textbf{\color{red} #1}}

% 统一
\newcommand{\mr}[1]{\mathrm{#1}}
\newcommand\LHS{\mathrm{LHS}}
\newcommand\RHS{\mathrm{RHS}}
%\newcommand\cd{\, \bm\cdot\, }
\newcommand\defeq{\coloneqq}

\numberwithin{equation}{section}
\newcommand{\case}[1]{\left\{\begin{aligned}
#1
\end{aligned}\right.}

% Brackets
\newcommand{\lb}[1]{\left\{#1\right\}}
\newcommand{\mb}[1]{\left[#1\right]}
\renewcommand{\sb}[1]{\left(#1 \right)}
\newcommand{\msb}[1]{\left[#1\right)}
\newcommand{\smb}[1]{\left(#1 \right]}

\newcommand{\bsb}[1]{\big(#1\big)}
\newcommand{\Bsb}[1]{\Big(#1\Big)}
\newcommand{\bbsb}[1]{\bigg(#1\bigg)}
\newcommand{\BBsb}[1]{\Bigg(#1\Bigg)}


% 一些缩写
\newcommand{\vp}{\varphi}
\newcommand{\ve}{\varepsilon}
\newcommand{\vk}{\varkappa}
\newcommand{\vn}{\varnothing}
\newcommand{\sbs}{\subset}
\newcommand{\sbse}{\subseteq}
\newcommand{\sps}{\supset}
\newcommand{\spse}{\supseteq}
\newcommand{\sm}{\setminus}
\newcommand{\ag}[1]{\begin{aligned}#1\end{aligned}}
\newcommand{\ol}[1]{\overline{#1}}
%\newcommand{\ul}[1]{\underline{#1}}
\newcommand{\wt}[1]{\widetilde{#1}}
\newcommand{\wh}[1]{\widehat{#1}}


% 分析
\DeclareMathOperator{\Ran}{\mathrm{Range}}
\DeclareMathOperator{\supp}{\mathrm{supp}}
\DeclareMathOperator{\Rl}{\mathrm{Re}}
\DeclareMathOperator{\Img}{\mathrm{Im}}
\DeclareMathOperator{\Lip}{\mathrm{Lip}}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\pv}{p.v.}
\DeclareMathOperator{\Spec}{\mathrm{Spec}}
\renewcommand{\ae}[1][]{\ #1\mathrm{a.e.}\ }
%\newcommand{\one}{\bm{\mathbbm 1}}
\newcommand\D{\mathrm D}
\newcommand\dr{\mathrm{d}}
\newcommand{\Leb}{\mathrm{Leb}}
\newcommand{\pa}{\partial^\alpha}

\newcommand{\nm}[1]{\left\|#1\right\|}
\newcommand{\gnm}[1]{\recbracket#1\recbracket}
\newcommand{\dv}[2][0]{\left.\frac{\dr}{\dr #2}\right|_{#2=#1}}
\newcommand{\pt}[2][]{\frac{\partial#1}{\partial #2}}%partial
\newcommand{\tv}[2]{\left. #1\right|_{#2}}%take values


\newcommand{\lto}[1]{\stackrel{#1}{\longrightarrow}}
\newcommand{\pair}[1]{\left\langle#1\right\rangle}
\newcommand{\abs}[1]{\left|#1\right|}

% 动力系统
\DeclareMathOperator{\Prob}{\mathrm{Prob}}
\newcommand{\Diff}{\mathrm{Diff}}
\newcommand{\Homeo}{\mathrm{Homeo}}
\newcommand{\gr}{\mathrm{gr}}
\newcommand{\Orb}{\mathrm{Orb}}
\newcommand{\reg}{\mathrm{reg}}

% 几何群论
\DeclareMathOperator{\Cay}{\mathrm{Cay}}
\DeclareMathOperator{\Ax}{\mathrm{Ax}}

% 概率
\DeclareMathOperator{\var}{var}
%\renewcommand{\P}{\bm{\mathrm P}}

% 代数与数论
\DeclareMathOperator{\spaned}{\mathrm{span}}
\DeclareMathOperator{\Tr}{\mathrm{tr}}
\DeclareMathOperator{\rank}{\mathrm{rank}}
\renewcommand{\mod}{\ \mathrm{mod}\ }
\newcommand{\Ad}{\mathrm{Ad}}
\newcommand{\ad}{\mathrm{ad}}
\newcommand\lcm{\mathrm{lcm}}
\newcommand{\Aut}{\mathrm{Aut}}
\newcommand{\End}{\mathrm{End}}
\newcommand{\id}{\mathrm{id}}
\newcommand{\Hom}{\mathrm{Hom}}
\newcommand{\diag}{\mathrm{diag}}
\newcommand{\Isom}{\mathrm{Isom}}

\newcommand{\GL}{\mathrm{GL}}
\newcommand{\SL}{\mathrm{SL}}
\newcommand{\PSL}{\mathrm{PSL}}
\newcommand{\SO}{\mathrm{SO}}
\newcommand{\Ct}{\mathbb{C}(\!(t)\!)}
\newcommand{\hyb}{\mathrm{hyb}}
\newcommand{\ord}{\mathrm{ord}}
\newcommand{\Di}{\mathbb{D}}

\newcommand{\lc}{\rm{lc}}
\newcommand{\lt}{\rm{lt}}

\newcommand{\mtx}[1]{\footnotesize{\mb{\setlength{\arraycolsep}{2.5pt}\begin{matrix}#1\end{matrix}}}}
\DeclareMathOperator{\Cl}{\mathrm{Cl}}

% 几何
\DeclareMathOperator{\Ind}{\mathrm{Ind}}
\newcommand{\Vol}{\mathrm{Vol}}
\DeclareMathOperator{\diam}{\mathrm{diam}}



% \mathcal字体
\newcommand{\cA}{\mathcal A}
\newcommand{\cB}{\mathcal B}
\newcommand{\cC}{\mathcal C}
\newcommand{\cD}{\mathcal D}
\newcommand{\cE}{\mathcal E}
\newcommand{\cF}{\mathcal F}
\newcommand{\cG}{\mathcal G}
\newcommand{\cH}{\mathcal H}
\newcommand{\cI}{\mathcal I}
\newcommand{\cJ}{\mathcal J}
\newcommand{\cK}{\mathcal K}
\newcommand{\cL}{\mathcal L}
\newcommand{\cM}{\mathcal M}
\newcommand{\cN}{\mathcal N}
\newcommand{\cO}{\mathcal O}
\newcommand{\cP}{\mathcal P}
\newcommand{\cQ}{\mathcal Q}
\newcommand{\cR}{\mathcal R}
\newcommand{\cS}{\mathcal S}
\newcommand{\cT}{\mathcal T}
\newcommand{\cU}{\mathcal U}
\newcommand{\cV}{\mathcal V}
\newcommand{\cW}{\mathcal W}
\newcommand{\cX}{\mathcal X}
\newcommand{\cY}{\mathcal Y}
\newcommand{\cZ}{\mathcal Z}

% \mathscr字体
\newcommand{\sA}{\mathscr A}
\newcommand{\sB}{\mathscr B}
\newcommand{\sC}{\mathscr C}
\newcommand{\sD}{\mathscr D}
\newcommand{\sE}{\mathscr E}
\newcommand{\sF}{\mathscr F}
\newcommand{\sG}{\mathscr G}
\newcommand{\sH}{\mathscr H}
\newcommand{\sI}{\mathscr I}
\newcommand{\sJ}{\mathscr J}
\newcommand{\sK}{\mathscr K}
\newcommand{\sL}{\mathscr L}
\newcommand{\sM}{\mathscr N}
\newcommand{\sN}{\mathscr N}
\newcommand{\sO}{\mathscr O}
\newcommand{\sP}{\mathscr P}
\newcommand{\sQ}{\mathscr Q}
\newcommand{\sR}{\mathscr R}
\newcommand{\sS}{\mathscr S}
\newcommand{\sT}{\mathscr T}
\newcommand{\sU}{\mathscr U}
\newcommand{\sV}{\mathscr V}
\newcommand{\sW}{\mathscr W}
\newcommand{\sX}{\mathscr X}
\newcommand{\sY}{\mathscr Y}
\newcommand{\sZ}{\mathscr Z}



% \mathbb 字体
\renewcommand{\AA}{{\mathbb A}}
\newcommand{\BB}{{\mathbb B}}
\newcommand{\CC}{{\mathbb C}}
\newcommand{\DD}{{\mathbb D}}
\newcommand{\EE}{{\mathbb E}}
\newcommand{\FF}{{\mathbb F}}
\newcommand{\GG}{{\mathbb G}}
\newcommand{\HH}{{\mathbb H}}
\newcommand{\II}{{\mathbb I}}
\newcommand{\JJ}{{\mathbb J}}
\newcommand{\KK}{{\mathbb K}}
\newcommand{\LL}{{\mathbb L}}
\newcommand{\MM}{{\mathbb M}}
\newcommand{\NN}{{\mathbb N}}
\newcommand{\OO}{{\mathbb O}}
\newcommand{\PP}{{\mathbb P}}
\newcommand{\QQ}{{\mathbb Q}}
\newcommand{\RR}{{\mathbb R}}
\renewcommand{\SS}{{\mathbb S}}
\newcommand{\TT}{{\mathbb T}}
\newcommand{\UU}{{\mathbb U}}
\newcommand{\VV}{{\mathbb V}}
\newcommand{\WW}{{\mathbb W}}
\newcommand{\XX}{{\mathbb X}}
\newcommand{\YY}{{\mathbb Y}}
\newcommand{\ZZ}{{\mathbb Z}}


% 黑体
\newcommand{\bA}{{\mathbf{A}}}
\newcommand{\bB}{{\mathbf{B}}}
\newcommand{\bC}{{\mathbf{C}}}
\newcommand{\bD}{{\mathbf{D}}}
\newcommand{\bE}{{\mathbf{E}}}
\newcommand{\bF}{{\mathbf{F}}}
\newcommand{\bG}{{\mathbf{G}}}
\newcommand{\bH}{{\mathbf{H}}}
\newcommand{\bI}{{\mathbf{I}}}
\newcommand{\bJ}{{\mathbf{J}}}
\newcommand{\bK}{{\mathbf{K}}}
\newcommand{\bL}{{\mathbf{L}}}
\newcommand{\bM}{{\mathbf{M}}}
\newcommand{\bN}{{\mathbf{N}}}
\newcommand{\bO}{{\mathbf{O}}}
\newcommand{\bP}{{\mathbf{P}}}
\newcommand{\bQ}{{\mathbf{Q}}}
\newcommand{\bR}{{\mathbf{R}}}
\newcommand{\bS}{{\mathbf{S}}}
\newcommand{\bT}{{\mathbf{T}}}
\newcommand{\bU}{{\mathbf{U}}}
\newcommand{\bV}{{\mathbf{V}}}
\newcommand{\bW}{{\mathbf{W}}}
\newcommand{\bX}{{\mathbf{X}}}
\newcommand{\bY}{{\mathbf{Y}}}
\newcommand{\bZ}{{\mathbf{Z}}}






% 一些哥特体
\newcommand{\fh}{\mathfrak h}
\newcommand{\fg}{\mathfrak g}
\newcommand{\fu}{\mathfrak u}
\newcommand{\fo}{\mathfrak o}
\newcommand{\fr}{\mathfrak r}
\newcommand{\fsu}{\mathfrak{su}}
\newcommand{\fgl}{\mathfrak{gl}}
\newcommand{\fsl}{\mathfrak{sl}}
\newcommand{\fsp}{\mathfrak{sp}}
\newcommand{\fso}{\mathfrak{so}}
\newcommand{\ft}{\mathfrak t}
\newcommand{\fz}{\mathfrak z}
\newcommand{\fs}{\mathfrak s}
\newcommand{\fM}{\mathfrak M}

\newcommand{\tr}{\mathrm{tr}}



\newcommand{\recbracket}{
\,
\begin{tikzpicture}[baseline]
\draw (0,-0.2em) -- (0em,0.8em) -- (0.2em,0.8em) -- (0.2em,-0.2em) -- (-0.02em,-0.2em);
\end{tikzpicture}
\,
}
\newcommand{\act}{
\,
\tikzset{every picture/.style={line width=0.07em}}
\begin{tikzpicture}[baseline]
\draw  (0,0) .. controls (0,0.8em) and (0.5em,0.8em) .. (0.5em,0);
\draw  (0.65em,0.15em) .. controls (0.56em,0.1em) and (0.52em,0.05em) .. (0.5em,0) .. controls (0.48em,0.05em) and (0.44em,0.1em) .. (0.35em,0.15em);
\end{tikzpicture}
\,
}

% WH use
%\newcommand{\dd}{\,\mathrm{d}}
\newcommand{\hFur}{h_\mathrm{F}}   % Furstenberg entropy
\newcommand{\hRW}{h_\mathrm{RW}}   % Random walk entropy
\newcommand{\dimH}{\dim_\mathrm{H}}% Hausdorff dimension
\newcommand{\unif}{u}     % uniform measure
\newcommand{\Zmodd}{[d]}           % Z mod d Z
\newcommand{\CCs}{\pi_0}             % Connected components
\newcommand{\len}[1]{\lvert#1\rvert}
\DeclareMathOperator{\Stab}{Stab}
\DeclareMathOperator{\Fix}{Fix}
%\DeclareMathOperator{\st}{st}      % cancellation
\DeclareMathOperator{\cl}{cl}      % cancellation
\DeclareMathOperator{\lcp}{lcp}      % longest common prefix


\renewcommand{\leq}{\leqslant}
\renewcommand{\geq}{\geqslant}




%LPX use
\renewcommand{\bf}[1]{\mathbf{#1}}
\renewcommand{\rm}[1]{\mathrm{#1}}
\renewcommand{\cal}[1]{\mathcal{#1}}
\newcommand{\bb}[1]{\mathbb{#1}}
\renewcommand{\frak}[1]{\mathfrak{#1}}
\newcommand{\bm}[1]{\mathbbm{#1}}
\newcommand{\dd}{\mathrm{d}}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\blue}[1]{{\color{blue}#1}}
\newcommand{\olive}[1]{{\color{olive}#1}}
\newcommand{\teal}[1]{{\color{teal}#1}}

\newcommand{\isep}{\mathrel{{.}\,{.}}\nobreak}
\newcommand{\ltr}{\mathrm{lt}_{\Re,M}'}
\newcommand{\plog}{\mathrm{plog}}

\def\R{\bb R}
\def\C{\bb C}
\def\P{\bb P}
\def\T{\bb T}
\def\B{\mathbbm 1}
\def\Z{\bb Z}
\def\Q{\bb Q}
\def\S{\bb S}
\def\N{\bb N}
\def\H{\bb H}
\def\E{\bb E}
\def\A{\bb A}
\def\D{\bb D}
\def\M{\bb M}

\def\calH{\cal H}
\def\calS{\cal S}
\def\calA{\cal A}
\def\calQ{\cal Q}
\def\calJ{\cal J}
\def\calF{\cal F}
\def\calO{\cal O}
\def\calP{\cal P}
\def\diag{\rm{diag}}
%\def\diam{\rm{diam}}
\def\SL{\rm{SL}}
\def\PGL{\rm{PGL}}
\def\PSL{\rm{PSL}}
\def\GL{\rm{GL}}
\def\SO{\rm{SO}}
\def\Id{\rm{Id}}
\def\Hom{\rm{Hom}}
\def\HA{\rm{HA}}

\def\bi{\bf i}
\def\bj{\bf j}
%\def\bU{\mathbf{U}}
%\def\bI{\mathbf{I}}

\def\Pkan{\P^{1,an}_k}

\DeclareMathOperator{\arccot}{\rm{arccot}}
\DeclareMathOperator{\sech}{\rm{sech}}
%\newcommand{\supp}{\rm{supp}}

%补丁
\renewcommand{\ve}{\epsilon}
























